Bandwidth Efficient and Rate-Matched Low-Density Parity-Check Coded Modulation

A new coded modulation scheme is proposed. At the transmitter, the concatenation of a distribution matcher and a systematic binary encoder performs probabilistic signal shaping and channel coding. At the receiver, the output of a bitwise demapper is fed to a binary decoder. No iterative demapping is performed. Rate adaption is achieved by adjusting the input distribution and the transmission power. The scheme is applied to bipolar amplitude shift keying (ASK) constellations with equidistant signal points and it is directly applicable to two-dimensional quadrature amplitude modulation (QAM). The scheme is implemented by using the DVB-S2 low-density parity-check (LDPC) codes. At a frame error rate of 1e-3, the new scheme operates within less than 1 dB of the AWGN capacity 0.5log2(1+SNR) at any spectral efficiency between 1 and 5 bits/s/Hz by using only 5 modes, i.e., 4-ASK with code rate 2/3, 8-ASK with 3/4, 16-ASK and 32-ASK with 5/6 and 64-ASK with 9/10.

==> Makefile <==
PROJECT=153dB_twocolumns
TMPFILES=*.aux *.bak *.bbl *.blg *.lof *.log *.toc *.lot *~ *.backup\
*.pfx *.ovp $(PROJECT)-pics.* $(PROJECT).dvi $(PROJECT).ps\
*.ind *.idx *.ilg *.gls *.glo *.glg *.acn *.acr *.alg *.ist *.out\
*.thm
ARXIVTMP=*.aux *.bak *.blg *.lof *.log *.toc *.lot *~ *.backup\
*.pfx *.ovp $(PROJECT)-pics.* $(PROJECT).dvi $(PROJECT).ps $(PROJECT).pdf *.bib .*.xml


default:
	pdflatex -shell-escape $(PROJECT).tex;

clean:
	rm -f $(TMPFILES);

clean_pdf:
	rm -f $(PROJECT).pdf;

final: clean clean_pdf
	pdflatex -shell-escape $(PROJECT).tex;
	pdflatex $(PROJECT).tex;
	bibtex $(PROJECT);
	pdflatex $(PROJECT).tex;
	pdflatex $(PROJECT).tex;
	pdflatex $(PROJECT).tex;
arxiv:
	rm -f $(ARXIVTMP);
	rm -rf .git;


